CROSS-JEM: Accurate and Efficient Cross-encoders for Short-text Ranking Tasks

Ranking a set of items based on their relevance to a given query is a core problem in search and recommendation. Transformer-based ranking models are the state-of-the-art approaches for such tasks, but they score each query-item independently, ignoring the joint context of other relevant items. This leads to sub-optimal ranking accuracy and high computational costs. In response, we propose Cross-encoders with Joint Efficient Modeling (CROSS-JEM), a novel ranking approach that enables transformer-based models to jointly score multiple items for a query, maximizing parameter utilization. CROSS-JEM leverages (a) redundancies and token overlaps to jointly score multiple items, that are typically short-text phrases arising in search and recommendations, and (b) a novel training objective that models ranking probabilities. CROSS-JEM achieves state-of-the-art accuracy and over 4x lower ranking latency over standard cross-encoders. Our contributions are threefold: (i) we highlight the gap between the ranking application's need for scoring thousands of items per query and the limited capabilities of current cross-encoders; (ii) we introduce CROSS-JEM for joint efficient scoring of multiple items per query; and (iii) we demonstrate state-of-the-art accuracy on standard public datasets and a proprietary dataset. CROSS-JEM opens up new directions for designing tailored early-attention-based ranking models that incorporate strict production constraints such as item multiplicity and latency.

==> sections/motivation.tex <==

\input{tables.tex/motivation_tables}
Our approach is based on designing a ranker that is capable of evaluating the entire set of items \(\sK_{\vq}\), given the query \(\vq\), as opposed to computing score for each ($\vq, \vk_j$) individually~\citep{FIXXX}. This design is motivated by two key insights from sponsored search applications, where the items to be retrieved are annotated with short descriptions that form the item set \(\sK_{\vq}\):
\begin{enumerate}[leftmargin=*]
    \item \textit{Sequence information is relatively less significant for scoring short-item text, when compared to token similarity matches}. We analyze the effect of the ordering/sequencing of the item text on classification accuracy using a cross-encoder model; and a train dataset consists of about 100M query-item pairs \((\vq,\vk)\), drawn from $\sQ_{tr} \times \sI_{tr}$, mined from proprietary search engine logs. Given \((\vq,\vk)\), we compare two cross-encoder \(\gE\) models: 1) $\gE_{CE}$: Standard cross-encoder scoring the pairs $(\vq, \vk)$, and 2) $\gE^{\prime}_{CE}$: Cross-encoder trained to score pairs $(\vq, \vk^{\prime})$, where the item $\vk^{\prime}$ is obtained by sorting the tokens in $\vk$ alphabetically.
  
The hypothesis is that, if the cross-encoders $\gE_{CE}$ and $\gE_{CE}^{\prime}$ have similar scoring accuracy, then the sequence ordering is relatively less informative for this task. While testing $\gE_{CE}^{\prime}$ is evaluated on \((\vq,\vk^{\prime})\) pairs \(\vk^{\prime}\) is drawn from $\sI_{te}$, with its tokens sorted alphabetically. Table~\ref{table_motivation}(a) shows how the variants perform on a test set of 10M pairs. We observe that, when the sequence information in \(\vk\) is discarded, both the mean average precision (MAP) and accuracy are within 1\% of the case when the sequence information is retained. 
\item \textit{The candidate items in the set \(\sK_{\vq}\) for a given query \(\vq\) have significant token overlap amongst themselves}. We train an ANCE~\citep{Xiong20} dense retriever on the same train set as above. For a query $\vq \in \sQ_{te}$, recall that $\sK_{\vq} = \{\vk_1, \vk_2, \ldots,\vk_{N}\}$ are the top $N$ (=100 in our experiments) items retrieved using ANCE. Let $\sT^L_{\vk_j}$ denote word-piece tokens in $\vk_j$ with a max-length of $L$. Let \(\sT_U\) denote the union of all tokens of items \(\vk_j \in \sK_{te}\). We compute the following two test-set statistics:
\begin{align}
    m~\text{(mean total tokens)} & =  \frac{1}{|\sQ_{te}|} \sum_{\vq \in \sQ_{te}} \left(\sum_{j=1}^{N} |\sT^L_{\vk_j}|\right),~\text{and} \\
    N_u~\text{(mean size of token union set \(\sT_U\))} & = \frac{1}{|\sQ_{te}|} \sum_{\vq \in \sQ_{te}} \left( \left| \bigcup_{j=1}^{N} \sT^L_{\vk_j}\right|\right).
\end{align}

Intuitively, \(m\) is the the sum of item token lengths on average, while \(N_u\) is the cardinaltity of the union set, averaged over the queries \(\vq\) for which the candidate items \(\sK_{\vq}\) were obtained. We hypothesize that, if the items \(\vk_i\) have significant overlap, \(m \gg N_u\). Table~\ref{table_motivation}(b) presents these statistics computed on about 400K $\vq \in \sQ_{te}$ as the maximum length  $L$ of the word-piece tokenizer is varied. 
The union size \(N_u\) is at least 5$\times$ smaller than \(m\), indicating high redundancy, and leading to our second insight. \par
\end{enumerate}


==> tables.tex/ablations_table.tex <==
\begin{table}
\centering
\scriptsize
\caption{Ablation study on Combiner Functions and Contribution of Clasifier Representations to \alg on N-Amazon-
1.3M dataset}
\label{tab:ablations}
% \resizebox{\linewidth}{!}{

    \begin{tabular}{l|ccc|ccc}
    \hline
    Method & \textbf{R@5} & \textbf{R@10} & \textbf{R@30} & \textbf{R@5} & \textbf{R@10} & \textbf{R@30} \\
    \hline
    \multicolumn{4}{c|}{\hspace{3.5 cm}Zero shot} & \multicolumn{3}{c}{One shot}\\ 
    \hline \hline
    Combiner - Sum & 30.36 & 38.13 & 49.29 & 30.74 & 38.71 & 50.36 \\ 
    Combiner - Weighted Sum  & 29.85 & 37.12 & 47.58 & 30.01 & 37.32 & 47.93 \\
    Combiner - Max  & 29.60 & 36.83 & 47.04 & 29.95 & 37.39 & 48.12 \\
    \alg & 31.22 & 39.03 & 50.13 & 31.68 & 39.72 & 51.14 \\
    \alg with Encoder Embeddings & 30.64 & 38.21 & 49.18 & 31.03 & 38.76 & 49.95 \\

    \hline
\end{tabular}
% }
\end{table}



==> tables.tex/dataset_stats.tex <==
\begin{table}[!t]
\centering
\footnotesize
\caption{Dataset Statistics.}
\label{table_dataset_statistics}
\vspace{-7pt}
\setlength{\tabcolsep}{2.0pt}
\begin{tabular}{l|ccccc}
\hline
\textbf{Dataset} & \textbf{\thead{\# Train}} & \textbf{\thead{\# \new \\ }} & \textbf{\thead{\# Gen \\ }} & \textbf{\# Train} & \textbf{\thead{\# \new}} \\
& \textbf{Qs} & \textbf{Test Qs} & \textbf{Test Qs} & \textbf{Items} & \textbf{Items}  \\
\hline
KeywordPrediction-5M* & 220,845,427  & 5,022,052 & 5,022,052 & 4,999,996 & 5,435,443 \\
N-AmazonTitles-1.3M & 2,225,354 & 624,830 & 970,237 & 1,174,739 & 130,526  \\
% N-ORCAS & 6,892,236 & 412,919 & 2,551,398 & 719,958 & 79,995 \\
N-Wikipedia-500K & 1,781,890 & 271,620 & 783,743 & 450,963 & 50,107 \\
\bottomrule
\end{tabular}
\end{table}

==> tables.tex/method_tables.tex <==
\begin{table}
\centering
\scriptsize
\caption{Performance when the associated items were (in a hypothetical scenario) revealed from the ground truth. Validation novel items were sampled from the N-Amazon-1.3M dataset to simulate these experiments. The accuracy degraded when the ground truth associations were progressively replaced by neighbors computed on the basis of similarity between the novel and seen item's encoder representations.}
\label{table_method1}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\textbf{Configuration} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5}   \\
\midrule
Ground truth associations & 33.80 & 22.66 & 17.62  \\
Replace 1 neighbor & 33.04 & 22.22 & 17.30  \\
Replace 2 neighbors & 32.30 & 21.73 & 16.93  \\
Replace 3 neighbors & 31.57 & 21.23 & 16.47  \\
\midrule
NGAME (no combiner) & 30.42 & 19.94 & 15.38   \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables.tex/results_internal.tex <==
\begin{table}[!t]
\centering
\scriptsize
\caption{Results on ads dataset}
\label{table_ads_main}
% \vspace{-7pt}
% \setlength{\tabcolsep}{4.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\textbf{Method} & \textbf{MAP@100} & \textbf{P@50} & \textbf{R@50}  & \textbf{AUC@50} \\
\midrule 
\alg & \textbf{97.48} & \textbf{45.76} & \textbf{99.07} & -\\
monoBERT & 98.42 & 45.87 & 99.21  & - \\
MEB & 84.38 & 42.94 & 94.65 & - \\

\hline
\end{tabular}
}
\end{table}


\begin{table}[!t]
\centering
\scriptsize
\caption{Results on ads dataset}
\label{table_ads_accuracy}
% \vspace{-7pt}
% \setlength{\tabcolsep}{4.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\textbf{Method} & \textbf{Negative Accuracy} & \textbf{Overall Accuracy} \\
\midrule 
\alg & \textbf{99.45} & \textbf{95.27} \\
monoBERT & 99.72 & 95.40 \\
MEB & 84.59 & 84.40 \\

\hline
\end{tabular}
}
\end{table}


\begin{table}[!t]
\centering
\scriptsize
\caption{Expert judges labeling results on KeywordPrediction-5M dataset}
\label{table_labeling}
% \vspace{-7pt}
% \setlength{\tabcolsep}{4.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c}
\toprule
\textbf{Method} & \textbf{\% of good quality predictions} \\
\midrule 
\alg - OneShot & 77.05 \\
\alg - ZeroShot & 73.16 \\
NGAME Encoder & 64.06 \\
\bottomrule
\end{tabular}}
\end{table}


\begin{table}[!t]
\centering
\scriptsize
\caption{Latencies required to perform different steps to get \alg representation for a \new item $y_u$. Steps 1, and 4 are done on a single V100 GPU, steps 2 and 3 on 96 CPU cores. All numbers are reported for batched operations.}
\label{table_latency}
\vspace{-7pt}
% \setlength{\tabcolsep}{4.5pt}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{l|c}
\toprule
\textbf{Step} & \textbf{Time (in $\mu s$)} \\
\midrule 
Calculate the embedding $\cE_{\vtheta}$ & 24 \\
Calculate encoder emb shortlist $S_{u}^{\vtheta}$ & 600 \\
Refine the shortlist using classifers to $S_{u}^{\vtheta}$ & 0.46 \\
Apply the Combiner function $\cC_{\vphi}$ & 0.3 \\
\bottomrule
\end{tabular}}
\end{table}

==> tables.tex/results_short_text_public.tex <==
\begin{table}[!t]
\scriptsize
    \caption{Results on public datasets with different algorithms.}
    \label{tab:results_repo_zero_shot_unseen}
    \vspace{-7pt}
\centering
\resizebox{\linewidth}{!}{
  \begin{tabular}{@{}l|ccc|ccc@{}}
  \toprule
   \multirow{2}{*}{Method}   & \multicolumn{3}{c}{\textbf{N-Amazon-1.3M}} & \multicolumn{3}{c}{\textbf{N-Wikipedia-500K}} \\ \cline{2-7}
    & \textbf{P@1} & \textbf{P@5} & \textbf{R@5}  & \textbf{P@1} & \textbf{P@5} & \textbf{R@5} \\ 
    \midrule
    & \multicolumn{6}{c}{Evaluation only on \new items} \\ 

    
    \hline \hline
    \alg-ZeroShot & \textbf{31.47} & \textbf{16.41} & \textbf{31.22} & \textbf{47.01} & \textbf{15.48} & \textbf{60.19} \\
    ANCE & 22.38 & 12.02 & 23.32 & 30.67 & 11.92 & 47.71 \\  
    NGAME Encoder & 30.42 & 15.38 & 29.40 & 46.96 & 15.10 & 58.91 \\
    SemSup-XC & 11.68 & 6.85 & 14.73 & 46.60 & 13.90 & 53.80 \\
    MACLR & 21.93 & 11.39 & 21.96 & 39.56 & 15.05 & 58.91\\
    ZestXML & 5.58 & 4.22 & 6.35 & 2.62 & 2.62 & 2.32\\
    TF-IDF  & 24.15 & 15.04 & 10.18 & 11.53 & 6.29 & 4.60 \\ 
         
    % \alg, ANCE, NGAME-enc, semsup, maclr, zestxml, tf-idf

    \midrule
    \alg-OneShot & \textbf{31.92} & \textbf{16.67} & \textbf{31.68} & \textbf{47.90} & \textbf{15.79} & \textbf{61.42} \\
    NGAME-OneShot (re-trained)  & 30.55 & 15.39 & 29.43 & 47.37 & 15.33 & 59.86 \\ 
    Semsup-XC-OneShot  & 13.96 & 6.98 & 15.49 & 46.25 & 13.77 & 53.67 \\  
    % MACLR-OneShot & - & - & - & - & - & - \\
    % ZestXML-OneShot & - & - & - & - & - & - \\
    NCM OneShot & 26.49 & 48.57 & 28.94 & 40.43 & 13.60 & 53.72 \\


    ADAM OneShot  & 20.80 & 11.71 & 25.73 & 39.79 & 13.39 & 52.97 \\

    \midrule
    & \multicolumn{6}{c}{Generalized evaluation} \\ 
    \hline
    \hline

    \alg & \textbf{45.81} & \textbf{35.61} & \textbf{23.10} & 81.79 & \textbf{46.10} & \textbf{61.69} \\     
    ANCE & 27.65 & 19.76 & 12.41 & 42.91 & 20.91 & 35.51\\
    NGAME Encoder & 45.14 & 34.72 & 22.58 & \textbf{81.86} & 45.38 & 60.96 \\
    Semsup-XC & 25.13 & 18.37 & 10.59 & 63.92 & 26.59 & 37.22 \\
    MACLR & 27.50 & 18.60 & 11.76 & 46.59 & 24.38 & 36.38 \\
    ZestXML & 22.87 & 26.79 & 39.71 & 45.15 & 54.31 & 59.32 \\
    % NGAME based (For unseen labels NCM is just label repr. for seen it will not just be label repr.) No NCM in unseen accuracies as it will be same as NGAME
    NCM  & 41.36 & 28.29 & 14.45 & 60.16 & 29.21 & 38.01 \\
    TF-IDF & 16.33 & 7.35 & 16.47 & 15.07 & 6.93 & 11.67 \\ 
    \midrule
    \alg-OneShot & \textbf{45.83} & \textbf{35.66} & \textbf{23.12} & 81.80 & \textbf{46.16} & \textbf{61.77} \\
    NGAME OneShot (re-trained) & 45.31 & 34.87 & 22.66 & \textbf{82.22} & 45.60 & 61.17 \\

    Semsup-XC OneShot & 22.48 & 15.66 & 10.03 & 60.97 & 25.40 & 36.16 \\
    % ZestXML OneShot  & - & - & - & - & - & - \\

    NCM OneShot  & 28.41 & 19.19 & 13.66 & 61.89 & 30.04 & 46.27 \\

    ADAM OneShot & 19.13 & 15.26 & 11.50 & 59.54 & 27.77 & 43.46 \\
        \bottomrule
\end{tabular}
}

\end{table}



==> tables.tex/results_wiki.tex <==
\begin{table}[!t]
\centering
\scriptsize
\caption{Results on N-Wikipedia-500K}
\label{table_wiki}
\resizebox{\linewidth}{!}{

    \begin{tabular}{l|cccccccc}
    \hline
    Method & \textbf{R@3} & \textbf{R@5} & \textbf{R@10} & \textbf{R@30} & \textbf{R@100} & \textbf{P@1} & \textbf{P@3} & \textbf{P@5} \\
    
    \hline
    \multicolumn{9}{c}{Evaluation only on \new items} \\ 
    \hline \hline
    
    
    
    
    % TF-IDF Unseen Unsupervised
    \alg-ZeroShot & 54.45 & 60.19 & 67.03 & 76.12 & 83.51 & 47.01 & 23.00 & 15.48  \\ 
    TF-IDF & 15.43 & 18.64 & 23.89 & 34.66 & 48.24 & 11.53 & 6.29 & 4.60 \\
    NGAME & 53.55 & 58.91 & 65.27 & 74.33 & 82.07 & 46.96 & 22.56 & 15.1 \\
    Semsup-XC & 50.38 & 53.80 & 57.08 & 60.01 & 61.03 & 46.60 & 21.46 & 13.90 \\
    ZestXML & 6.86 & 9.95 & 14.73 & 21.63 & 25.55 & 2.62 & 2.62 & 2.32 \\
    MACLR & - & - & - & - & - & - & - & -  \\
    
    
    \midrule
    
    \alg-OneShot  & 55.38 & 61.42 & 68.69 & 78.08 & 85.5 & 47.90 & 23.39 & 15.79  \\
    Semsup-XC OneShot  & 50.21 & 53.67 & 57.04 & 60.04 & 61.02 & 46.25 & 21.24 & 13.77  \\
    NGAME OneShot & 54.42 & 59.86 & 66.37 & 75.28 & 82.85 & 47.37 & 22.92 & 15.33  \\

    NCM OneShot & 48.03 & 53.72 & 60.94 & 71.26 & 80.22 & 40.43 & 19.97 & 13.60  \\
    
    \hline
    \multicolumn{9}{c}{Generalized Evaluation} \\ 
    \hline \hline
    
    % TF-IDF GZSXC Unsupervised
    \alg & 52.58 & 61.69 & 70.75 & 80.24 & 87.20 & 81.79 & 60.55 & 46.10  \\
    TF-IDF & 9.49 & 11.67 & 14.79 & 20.87 & 30.10 & 15.07 & 9.19 & 6.93 \\
    NGAME & 52.24 & 60.96 & 69.58 &  78.67 & 85.50 & 81.86 & 60.13 & 45.38\\
    Semsup-XC & 34.22 & 37.22 & 39.37 & 40.72 & 41.10 & 63.92 & 38.84 & 26.59 \\
    ZestXML & 32.24 & 38.01 & 45.15 & 54.31 & 59.32 & 60.16 & 39.33 & 29.21 \\
    NCM  & 38.88 & 45.69 & 54.20 & 66.13 & 76.54 & 60.51 & 39.50 & 29.58 \\

    \hline
\end{tabular}}
\end{table}


